Almost Optimal Time Lower Bound for Approximating Parameterized Clique, CSP, and More, under ETH

The Parameterized Inapproximability Hypothesis (PIH), which is an analog of the PCP theorem in parameterized complexity, asserts that, there is a constant $\varepsilon> 0$ such that for any computable function $f:\mathbb{N}\to\mathbb{N}$, no $f(k)\cdot n^{O(1)}$-time algorithm can, on input a $k$-variable CSP instance with domain size $n$, find an assignment satisfying $1-\varepsilon$ fraction of the constraints. A recent work by Guruswami, Lin, Ren, Sun, and Wu (STOC'24) established PIH under the Exponential Time Hypothesis (ETH). In this work, we improve the quantitative aspects of PIH and prove (under ETH) that approximating sparse parameterized CSPs within a constant factor requires $n^{k^{1-o(1)}}$ time. This immediately implies that, assuming ETH, finding a $(k/2)$-clique in an $n$-vertex graph with a $k$-clique requires $n^{k^{1-o(1)}}$ time. We also prove almost optimal time lower bounds for approximating $k$-ExactCover and Max $k$-Coverage. Our proof follows the blueprint of the previous work to identify a "vector-structured" ETH-hard CSP whose satisfiability can be checked via an appropriate form of "parallel" PCP. Using further ideas in the reduction, we guarantee additional structures for constraints in the CSP. We then leverage this to design a parallel PCP of almost linear size based on Reed-Muller codes and derandomized low degree testing.

==> improve/linear.tex <==
\section{Linear Part}

\xr{Temporarily put everything here. Should move some to preliminary.}

\begin{definition}[\textsc{Zero-on-SubHypercube} Problem]
    For a finite field $\mathbb F$, its sub-field $\mathbb H$, and an integer $d$, an $(\mathbb F,\mathbb H, m, d)$ instance of the \textsc{Zero-on-SubHypercube} problem is the class of degree-$d$ $m$-variate polynomials over $\mathbb F$, such that $\forall x_1,\ldots,x_m \in \mathbb H$, $f(x_1,\ldots,x_m) = 0$. In other words, $f \equiv 0$ on $\mathbb H^m$.
\end{definition}


\begin{definition}[PCPP for \textsc{Zero-on-SubHypercube}]
    We say $\mathcal P$ is a $(q,r,s)$-PCPP verifier for the \textsc{Zero-on-SubHypercube} instance $(\mathbb F,\mathbb H, m, d)$, if it takes as input the truth table of an $m$-variate polynomial $f$ over $\mathbb F$ together with a proof $\pi$, tosses $r$ random coins, makes $q$ queries on the truth table, and then decides to accept or reject.
    \begin{itemize}
        \item If $f$ is of degree at most $d$ and  equals 0 on $\mathbb H^m$, then there is a proof $\pi$ which always makes $\mathcal P$ accept.
        \item Otherwise for any proof $\pi$, $\mathcal P$ accepts with probability at most $s$.
    \end{itemize}
\end{definition}

We remark that the size of the proof $\pi$ can be bounded by $q \cdot 2^r$, since that's the most number of positions $\mathcal P$ is possible to access.

\begin{lemma}[]\label{lem:zero-prop}
    \xr{Put the reference of the construction here.}
\end{lemma}

\xr{Should somehow agree ``a vector of polynomial'' or ``a polynomial vector''?}


In this section, we design a parallel PCP of proximity for the linear part of a \svcsp{}.

Recall that the linear part of a \svcsp{} instance $G=(V,E,\Sigma,\{\Pi_e\}_{e \in E})$ has the following properties:\vg{Perhaps we can use $f_i,g_i$ instead of $x_i,y_i$ as we will soon think of these as multivariate polynomials? But not a big deal either way}
\begin{itemize}
    \item $V=\{x_1,\ldots,x_k\} \dot\cup\{y_1,\ldots,y_k\}$.
    \item $\Sigma=\mathbb F^t$ is a $t$-dimensional vector space over a finite field $\mathbb F$.
    \xr{Here use $t$ instead.}
    \item $E=\{(x_i,y_i)\}_{i \in [k]}$, and for each $i \in [k]$, we are constraining $y_i = A_i \cdot x_i$.\vg{Weren't we applying $A_i$ to the tail per definition}
\end{itemize}

Let $\mathbb H$ be a sub-field of $\mathbb F$ and let $d=m \cdot |\mathbb H|$ with $m$ to be determined. In the following, we associate $[k]$ with $\mathbb H^m$, and use $x(i) \in \mathbb F^d$ (respectively, $y(i) \in \mathbb F^d, A(i) \in \mathbb F^{d \times d}$) for an index $i=(i_1,\ldots,i_m) \in \mathbb H^d$ to denote the variables and the constraint matrices. We can naturally interpolate degree-$d$ polynomial vectors/matrices of $x,y,A$, and thus extend them to $\mathbb F^d$. The problem then becomes:

\begin{itemize}
    \item Check whether $y(i) = A(i) \cdot x(i)$ for every $i=(i_1,\ldots,i_m) \in \mathbb H^m$, where $x(\cdot ),y(\cdot )$ are vectors of degree-$d$ polynomials, and $A(\cdot)$ is a matrix of degree-$d$ polynomials. In other words, for every $u,v \in [t]$, $x(\cdot )[u], y(\cdot)[u]$ and $A(\cdot)[u,v]$ are all degree-$d$ polynomials over $\mathbb F^m$.
\end{itemize}





Define a vector of polynomials $z(\cdot)$ by letting $z(i) = y(i)-A(i)\cdot x(i)$ for every $i \in \mathbb F^m$. It's easy to see each entry of $z$ is a degree-$2d$ polynomial over $\mathbb F^m$. The goal is then to prove $z(\cdot)$ evaluates to $\vec 0$ on the sub-hypercube $\mathbb H^m$. We then construct our parallel PCPP verifier $\mathcal P$, which takes as input the truth tables of $x(\cdot),y(\cdot),z(\cdot)$, and make the following queries:

\begin{itemize}
    \item Use the parallel low-degree test to check whether $x(\cdot),y(\cdot)$ and $z(\cdot)$ are all close to vectors of polynomials.
    \item Apply \Cref{lem:zero-prop} with the same randomness on all $t$ vector-entries of $z(\cdot)$. Reject if for any $j \in [t]$, $z(\cdot)[j] \not\equiv 0$ on $\mathbb H^m$.
    \item Pick a random point $i=(i_1,\ldots,i_m) \in \mathbb F^m$, reject if $z(i) \neq y(i) - A(i) \cdot x(i)$.
\end{itemize}

\xr{
Parameter calculation:
$$\left\{\begin{aligned}
    |\mathbb H|^m & \ge k \\
    d & = m |\mathbb H| \\ 
    |\mathbb F| & \ge 6m \cdot d = 6m^2 |\mathbb H|\text{ (for low-degree test, \Cref{thm:derand_augpldt_detail})}
\end{aligned}\right.$$

Let $m = (\log k)^{\mu}$ for some $0 < \mu < 1$, then 

$$\left\{\begin{aligned}
    |\mathbb H| & = k^{1/m} = 2^{(\log k)^{1-\mu}} \\
    |\mathbb F|^m  & = k \cdot (6m^{2})^m \approx k \cdot 2^{2\mu (\log k)^{\mu}\log \log k} = k^{1+o(1)} \\
    \text{proof alphabet size }N & = |\mathbb F|^{n\cdot \log k/k} = 2^{n\cdot \text{poly}\log (k)/k}
\end{aligned}\right.$$

Can say there's no $N^{k^{1-o(1)}}$ algorithm.
}
\vg{Can also take $m = \log k/(\log\log k)^2$ and $|\mathbb H| = (\log k)^{\log \log k}$. In any case the big loss will be the from the near-linear PCP which has $2^{\sqrt{\log k}}$ blow-up.}
\xr{In fact we need $|\mathbb F| \ge \Omega(m \cdot d)$ instead of $|\mathbb F| \ge \Omega(d)$ due to the low-degree test, which are forgotten in our last discussion :-(. But anyway it seems the above parameters still work.}
\begin{comment}

We have the following ``zero-propagation'' protocol from e.g. \cite{?}.\vg{Isn't sum check protocol the name that's used for this?}

Define vectors of polynomials $z_0,\ldots,z_m$, where $z_0=z$, and 
\begin{equation}\label{eq:def-z}
    z_j(i_1,\ldots,i_m) = \sum_{a \in \mathbb H} z_{j-1} (i_1,\ldots,i_{j-1}, a, i_{j+1},\ldots,i_m)\cdot i_j^a.
\end{equation}

It's easy to see $z_0,\ldots,z_m$ are all vectors of degree-$d$ polynomials.

\begin{lemma}\label{lem:zero-prop}
    For every $j \in [m]$,
    $$
    z_{j-1}(\cdot) \equiv \vec 0\text{ over }\mathbb F^{j-1}\times \mathbb H^{m-j+1} \Leftrightarrow z_{j}(\cdot) \equiv \vec 0 \text{ over } \mathbb F^j \times \mathbb H^{m-j}.
    $$
\end{lemma}

\begin{proof}[Proof of \Cref{lem:zero-prop}]
$\Rightarrow$: For every $i_1,\ldots,i_j \in \mathbb F$ and $i_{j+1},\ldots,i_m \in \mathbb H$, by definition, $z_j(i_1,\ldots,i_m)$ evaluates to the sum of $|\mathbb H|$ terms $z_{j-1}(i_1,\ldots,i_{j-1},a,i_{j+1},\ldots,i_m)\cdot i_j^a$. However, the coefficient of each term is $\vec 0$ by assumption. Thus, $z_j(\cdot ) \equiv \vec 0$ over $\mathbb F^j \times \mathbb H^{m-j}$.

$\Leftarrow$: Prove by contradiction. Suppose for some $i_1,\ldots,i_{j-1} \in \mathbb F$ and $i_j,\ldots i_m \in \mathbb H$, $z_{j-1}(i_1,\ldots,i_m) \neq \vec 0$. Then fix $i_1,\ldots,i_{j-1},i_{j+1},\ldots,i_m$ and fix $a$ to be the value of $i_j$. The term $$z_{j-1}(i_1,\ldots,i_{j-1},a,i_{j+1},\ldots,i_m) \cdot i_j^a$$ is not a (vector of) zero-polynomial of $i_j$. Then so is $$\sum_{a \in \mathbb H} z_{j-1}(i_1,\ldots,i_{j-1},a,i_{j+1},\ldots,i_m) \cdot i_j^a$$ as a polynomial of $i_j$. Given that the above has degree at most $|\mathbb H|$ over $i_j$, it cannot evaluate to zero for all $i_j \in \mathbb F$. Therefore, $z_j \not\equiv \vec 0$ over $\mathbb F^j \times \mathbb H^{m-j}$.
\end{proof}

Given \Cref{lem:zero-prop} holds, $z(\cdot) \equiv \vec 0$ over $\mathbb H^m$ is equivalent to $z_m(\cdot) \equiv \vec 0$ over $\mathbb F^m$. 

The protocol is then as follows. We ask the prover to provide the truth tables of $x(\cdot), y(\cdot)$ and $ z_0(\cdot), \ldots, z_m(\cdot)$ over $\mathbb F^m$, and perform the following checks:
\begin{enumerate}
    \item Check whether $x(\cdot), y(\cdot)$ and each of the $z_j(\cdot)$'s are vectors of degree-$d$ polynomials.
    \item Check whether $z_0(\cdot) = y(\cdot) - A(\cdot) \cdot x(\cdot)$ holds at a random point $(i_1,\ldots,i_m) \in \mathbb F^m$.
    \item Check whether for each $j \in [m]$, \Cref{eq:def-z} holds. This is done by picking a random point $i^{(j)}=(i^{(j)}_1,\ldots,i^{(j)}_{m})\in \mathbb F^m$ for each $j$ and check whether the $j$-th equation holds.
    \item Check whether $z_m$ is a (vector of) zero-polynomial by checking whether it evaluates to $\vec 0$ at a random point in $\mathbb F^m$.
\end{enumerate}
\end{comment}

==> improve/pcpp-ldt.tex <==
\newcommand{\ldtquery}{??_1}
\newcommand{\ldtrandom}{(m+O(1))\log |\mathbb F| + O(\log \log |\mathbb F|+\log m) }
\newcommand{\ldtdelta}{\delta}
\newcommand{\ldtdeltaupp}{??_2}
\newcommand{\ldtrobust}{??_3}
\newcommand{\ldteps}{??_4}
\newcommand{\problemldt}{{\sc ParallelLDT}}

\subsection{PCPP for Low Degree Test}
\label{sec:pcpp-ldt}
In this part, we transform the line-point test~(\Cref{sec:lowdeg}) into a constant-query robust PCPP, by composing the parallel ``line-point'' test with Had. We first formalize the parallel low-degree test in a pair language.

\begin{definition}
\label{def:ldt-pair}
Given the dimension $t$, we define the pair language \problemldt{} over $\{0,1\}^t$ as follows. It consists of all pairs of words $((1^{\mathbb F}, 1^d, 1^m, 1^k), T)$ where:
\begin{itemize}
    \item ${\rm char}\ \mathbb F=2$, $|\mathbb F|\ge 6md$ and $m\le 2^{-100}\cdot\frac{|\mathbb F|}{\log |\mathbb F|}$.
    \item $T$ is a codeword of $(k, \mathbb F, m, d, t)$-parallel concatenated RM Code. 
\end{itemize}
In the following, we treat $T$ as a map $|\mathbb F|^m\times [3\log |\mathbb F|]\to \{0,1\}^t$.
\end{definition}

\begin{theorem}
\label{thm:pcpp-ldt}
For every $\delta\le \ldtdeltaupp$, there exists a $(\ldtquery, \ldtrandom, \ldtrobust, \ldtdelta, \ldteps)$-robust PCPP verifier for \problemldt{}.
\end{theorem}

\begin{proof}
We prove this theorem by proof composition.

\paragraph{Outer Verifier} The outer verifier $\mathcal P_{out}$ directly applies the parallel codeword testing for the concatenated RM Code~(\Cref{thm:derand_pldt}). By \Cref{thm:derand_pldt}, the outer verifier tosses $m\log |\mathbb F| + O(\log \log |\mathbb F|+\log m)$ random coins and makes $O(|\mathbb F|\log |\mathbb F|)$ queries. For every  proximity parameter $\delta_{out}\le ??_1$, it has the perfect completeness, and the $O(\delta_{out})$-robust soundness $1-\Omega(\delta_{out})$. Furthermore, all tests of the outer verifier check whether the queried $O(|\mathbb F|\log |\mathbb F|)$ bit-vectors form a codeword of $(\mathbb F, 1, d, t)$-parallel concatenated RM Code.

\paragraph{Inner Verifier} Note that all tests performed by the outer verifier can be checked by a circuit $C$ of size $|\mathbb F|^{O(1)}$. Thus, we invoke \Cref{thm:pcpp-main} to get an inner $(??,??,??,??,??)$-robust PCPP verifier $\mathcal P_{in}$. The theorem follows by instantiating the composition theorem~(\Cref{thm:comp}) for $\mathcal P_{out}\circ \mathcal P_{in}$.

\end{proof}

==> improve/pcpp-lineq.tex <==
\subsection{PCPP for Linear Equations}


==> improve/polypcpp.tex <==
\newcommand{\qval}{??_1}
\newcommand{\rhoval}{??_2}
\newcommand{\rval}{??_3}
\newcommand{\epsval}{??_4}
\newcommand{\duppval}{??_5}
\newcommand{\pcrm}{{\sf PCRM}^{\odot t}}

\section{PCPP Constructions}
\label{sec:pcpp}

\subsection{PCPPs for \pcircuit{}}
\label{sec:pcpp-pcircuit}

In this part, we design robust PCPP for \pcircuit{} (\Cref{def:pcircuit}).
\begin{theorem}
\label{thm:pcpp-main}
For every $\delta \le \duppval$, there exists a $(\qval,\rval,\rhoval,\delta,\epsval)$-PCPP verifier for \pcircuit{}.
\end{theorem}

We prove this theorem following the spirit of~\cite{almss98}. We first construct robust PCPPs with polylog queries.
\begin{proposition}
\label{prop:pcpp-pcircuit-polylog}
For every $\delta \le \duppval$, there exists a $(\qval,\rval,\rhoval,\delta,\epsval)$-PCPP verifier for \pcircuit{}.
\end{proposition}

\begin{proof}[Proof of \Cref{prop:pcpp-pcircuit-polylog}]
    Below, we fix the dimension $t$, and a pair word $(C,x)$ over the alphabet $\{0,1\}^t$.

    Let $m = \frac{\log k}{\log \log k}$, $H = k^{1/m} = \log k$, and $\mathbb F$ to be a field with characteristic 2 and size $\ge 6m^2H$. Note that $\mathbb F\le \frac{12\log^3k}{\log \log^2 k}$, and the choice of $m,d,\mathbb F$ fulfills the parameter requirements of the $(k,\mathbb F,m,mH,t)$-parallel concatenated RM code $\pcrm(\cdot): (\{0,1\}^t)^k\to (\{0,1\}^t)^{|\mathbb F|^m\cdot 3\log |\mathbb F|}$, where we further denote $\ell$ as the output length. As a result, we can use this code to encode $x$ to $\hat{x}:=\pcrm(x)$. $\hat{x}$ has the length $k^{O(1)}$.

    Next, we construct a circuit $C'$ over $\ell$-bit inputs. For the given input $\hat{y}$, $C'(\hat{y})$ checks whether $\hat{y}$ is a codeword of $\pcrm$, and its decoding result $y\in (\{0,1\}^t)^k$ parallel satisfies the original ciruict $C$. Since all checks can be done in polynomial time, the circuit size $|C'|$ is no more than $|C| + \ell^{O(1)} = |C| + k^{O(1)}$.

    Thus, by \Cref{thm:almss}, there exists a PCPP verifier $\mathcal P_{ckt}$ for {\sc CktVal}, with the parameters as \Cref{thm:almss}. Below, we parallelize $\mathcal P_{ckt}$ and obtain a robust PCPP verifier $\mathcal P$ for \pcircuit{}.

    The auxiliary proof for $\mathcal P$ consists of three parts. 
    \begin{itemize}
        \item The first part is denoted by $x_{{\rm copy}}$, for each $i\in [k]$, $x_{{{\rm copy}},i}$ is supposed to be a word of length $[3|\mathbb F|\log |\mathbb F|]$ that simply copies $x_i$ with $3|\mathbb F|\log |\mathbb F|$ times. This is used to ensure the robustness of the testing.
        \item The first part is denoted by $\hat{\pi}$, which is supposed to be $\hat{x}$. We may treat $\hat{\pi}$ as map from $\mathbb F^m\times [3\log |\mathbb F|]\to \{0,1\}^t$. For each $i\in [k]$, we denote $p_i\in \mathbb F^m$ as the position of $\hat{x}$ that stores ${\rm ECC}(x_i)$.
        \item The second part is denoted by $\pi_{ckt}$. $\pi_{ckt}$ has the alphabet $(\{0,1\}^t)$ and the length $\ell^{O(1)} = k^{O(1)}$. For each $i\in [t]$, $(\pi_{ckt,1}[i], \pi_{ckt,2}[i],\dots,\pi_{ckt,|\pi_{ckt}|}[i])$ is supposed to be the auxiliary proof for $\mathcal P_{ckt}$ to check whether $(\hat{x}_1[i],\dots,\hat{x}_l[i])$ satisfies the circuit $C'$.
    \end{itemize}

    Below, we describe the testing procedure. $\mathcal P$ executes each of the following four tests with equal probability $\frac14$.
    \begin{itemize}
        \item $\mathcal P$ invokes the randomized codeword testing for parallel concatenated RM code, on $\hat{\pi}$. This part tests whether $\hat{\pi}$ is a codeword of $\pcrm$.
        \item $\mathcal P$ simulates $\mathcal P_{ckt}$ on $\hat{\pi}\circ \pi_{ckt}$, for all coordinates. In detail, $\mathcal P$ tosses random coins as $\mathcal P_{ckt}$ does,         
        and probes all indices of $\hat{\pi}\circ \pi_{ckt}$ queried by $\mathcal P_{ckt}$. Given that $\mathcal P$ makes $q$ queries and the query result is $a\in (\{0,1\}^t)^q$, $\mathcal P$ accepts if and only if for every $i\in [t]$, $\mathcal P_{ckt}$ accepts $a_1[i], a_2[i], \dots, a_q[i]$. This part checks whether $\hat{\pi}$ parallel satisfies the circuit $C'$.
        \item $\mathcal P$ randoms $i\in [k], d\in \mathbb F^m\setminus\{0\}$, and queries all $\hat{\pi}(p_i + ad, \cdot)$ for each $a\in \mathbb F$. $\mathcal P$ checks whether for every $a\in \mathbb F$, $\hat{\pi}(p_i + ad, \cdot)$ is a codeword of ${\rm ECC}(\cdot)$, and the sub truth table $q(a):={\rm Dec}(\hat{\pi}(p_i+ad,\cdot))$ is a truth table of some $m$-variate polynomial with parallel degree $\le mH$, and $q(0)\in \{0,1\}$. Then, $\mathcal P$ reads all $3|\mathbb F|\log |\mathbb F|$ bits of $x_{{\rm copy},i}$, and checks whether all these bit-vectors equal $q(0)$.
        \item $\mathcal P$ randomes $i\in [k]$ and $j\in [3|F|\log |\mathbb F|]$ and checks whether $x_i$ equals $x_{{\rm copy},i,j}$.
    \end{itemize}

    First, we count the number of queries. By \Cref{thm:derand_pldt}, the first part makes $O(|\mathbb F|\log |\mathbb F|) = (\log k)^{O(1)}$ queries. By \Cref{thm:almss}, the second part makes $(\log k)^{O(1)}$ queries. The third part makes $3|\mathbb F|\log |\mathbb F| = (\log k)^{O(1)}$ queries. Thus, the verifier $\mathcal P$ makes $(\log k)^{O(1)}$ queries.

    Second, we upper bound the number of random bits used by $\mathcal P$. By \Cref{thm:derand_pldt}, the first part costs $O(m\log |\mathbb F|) = O(\log k)$ random bits. By \Cref{thm:almss}, the second part costs $O(\log k)$ random bits, and the third part costs $\log k + m\log |\mathbb F| = O(\log k)$ random bits. Thus, $\mathcal P$ costs $(\log k)$ random bits.

    Then, we analyze the completeness. If $x$ parallel satisfies $C$, then we set $x_{{\rm copy}}$ as copies of $x$, $\hat{\pi}$ as $\pcrm(x)$. Note that $\hat{\pi}$ parallel satisfies $C'$, we can further set $\pi_{ckt}$ as the auxiliary proof that $\hat{\pi}$ parallel satisfies $C'$. For the first part, since $\hat{\pi}$ is a codeword, by the completeness of \Cref{thm:derand_pldt}, the verifier always accepts. For the second part, since $\hat{\pi}$ parallel satisfies $C'$, by the completeness of $\mathcal P_{ckt}$~(\Cref{thm:almss}), the verifier always accepts. For the third part, since $\hat{\pi}$ is a codeword of $\pcrm$, all $\hat{\pi}(p_i+ad,\cdot)$ is a codeword of ${\rm ECC}$, and the truth table is $q(a)$ is always a polynomial with parallel degree $\le md$. Furthermore, since $x_{{\rm copy}, i, \cdot}$ is a repetition of $x_i$, $q(0)$ always equals $x_{{\rm copy},i,\cdot}$. Thus, the verifier always accepts. For the fourth part, $\mathcal P$ always accepts by the construction of $x_{{\rm copy}}$.

    Finally, we analyze the robust soundness. Suppose $x$ is $\delta$-far from any $x'$ that parallel satisfies $C$. Below, we show that the verifier has $\frac{\delta}{2}$-robust soundness $1-\Omega(\delta)$ by the following chain of claims. We defer the proof of these claims at the end of this section.

    \begin{claim}
    \label{claim:1}
        $\hat{\pi}$ is $\delta$-close from some codeword of $\pcrm(x)$, otherwise $\mathcal P$ has $\frac{\delta}{2}$-robust soundness $\le 1-\Omega(\delta)$.
    \end{claim}

    By~\Cref{claim:1}, we can assume $\hat{\pi}$ is $\delta$-close to some codeword $\pi^*$ of $\pcrm(x)$.

    \begin{claim}
    \label{claim:2}
        $\pi^*$ parallel satisfies $C'$, otherwise $\mathcal P$ has $\frac{\delta}{2}$-robust soundness $\le 1-\Omega(\delta)$.
    \end{claim}

   By~\Cref{claim:2}, we can further assume $\pi^*$ parallel satisfies $C'$. Let $x^*$ to be the word that $\pi^* = \pcrm(x^*)$. By the construction of $C'$, we have that $x^*$ parallel satisfies $C$. Define $B$ as the set of all indices $i\in [k]$ such that $\Pr_{j\in [3|\mathbb F|\log |\mathbb F|]}[x_{{\rm copy},i,j}\ne x_i^*]\ge \frac12$.

   \begin{claim}
   \label{claim:3}
       $\Pr_{i\in [k]}{[i\in B]}\le \frac{\delta}{2}$, otherwise $\mathcal P$ has $\frac{\delta}{2}$-robust soundness $\le 1-\Omega(\delta)$.
   \end{claim}

   By~\Cref{claim:3}, we can assume that $\Pr_{i\in [k]}{[i\in B]}\le \frac{\delta}2$. By assumption, $\Delta(x,x^*)\ge \delta$. Thus, there exists at least $\frac{\delta}{2}$-fraction of $i$ such that: (1) $x_i\ne x_i^*$, and (2) $i\notin B$. For each of such $i$, $x_{{\rm copy}, i, j} = {\rm Dec}(\pi^*(p_i, \cdot)) = x_i^*\ne x_i$ for at least a half proportion of $j$. As a result, the fourth part of the tests has $\frac{1}{2}$-robust soundness $1-\frac{\delta}{4}$, since it only queries two locations. Thus, $\mathcal P$ has $\frac{\delta}{2}$-robust soundness $1-\Omega(\delta)$.
\end{proof}

The main PCPP construction~(\Cref{thm:pcpp-main}) follows by composing robust PCPPs designed above.

\begin{proof}[Proof of \Cref{thm:pcpp-main}]
Define $\mathcal P_{\rm log}$ as the verifier obtained from~\Cref{prop:pcpp-pcircuit-polylog}, and $\mathcal P_{\rm exp}$ as the verifier obtained from~\Cref{thm:pcpp-exp-circuit}. Then the theorem follows by the composition $\mathcal P_{\rm log}\circ \mathcal P_{\rm log}\circ \mathcal P_{\rm exp}$.
\end{proof}

Below, we prove all auxiliary claims used to prove \Cref{prop:pcpp-pcircuit-polylog}.

\begin{proof}[Proof of \Cref{claim:1}]
If $\hat{\pi}$ is $\delta$-far from any codeword of $\pcrm(x)$, recall that $\mathcal P$ invokes the codeword testing with probability $\frac14$. Thus, by the robust soundness of \Cref{thm:derand_pldt}, the verifier has $\frac{\delta}{2}$-robust soundness $\le 1-\Omega(\delta)$.
\end{proof}
\begin{proof}[Proof of \Cref{claim:2}]
Suppose for some $i\in [t]$, $\pi_1^*[i], \dots \pi_{\ell}^*[i]$ does not satisfy $C'$. Since $\Delta(\hat{\pi},\pi^*)\le \frac{\delta}{2}$, we have that: $$\Delta(\hat{\pi}_1[i]\cdots \hat{\pi}_{\ell}[i],\pi_1^*[i]\cdots \pi_{\ell}^*[i])\le \Delta(\hat{\pi},\pi^*)\le \frac{\delta}{2}.$$ By the construction of $C'$, $\hat{\pi}_1[i]\cdots \hat{\pi}_{\ell}[i]$ is $(1-\frac{mH}{|\mathbb F|}-\frac{\delta}{2})$-far from any satisfying assignment of $C'$. By the robust soundness of $\mathcal P_{ckt}$ (\Cref{thm:almss}), the second part of the tests has $\Omega(1)$-robust soundness at most $1-\Omega(1)$. Certainly, these test has $\frac{\delta}{2}$-robust soundness at most $1-\Omega(\delta)$. Since the second part of tests is picked with probability $\frac{1}{4}$, we have that, if $\pi^*$ does not parallel satisfy $C'$, $\mathcal P$ has $\frac{\delta}{2}$-robust soundness $\le 1-\Omega(\delta)$.
\end{proof}
\begin{proof}[Proof of \Cref{claim:3}]
    Suppose $\Pr_{i\in [k]}[i\in B]\ge \frac{\delta}2$. Consider the random line $Y = \{ad+p_i|a\in \mathbb F\}$, and define $Y_a$ as the random variable $ad+p_i$. Consider the following two events.
    \begin{enumerate}[label=\textbf{(E\arabic*)}]
        \item \label{itm:polypcpp:e1} $\Delta(\hat{\pi}|_Y, \pi^*|_Y)\le 4\Delta(\hat{\pi},\pi^*)$.
        \item \label{itm:polypcpp:e2} $i\in B$.
    \end{enumerate}

    First, we lower bound $Pr[E_1\land E_2]$. Note that $\Pr[E_1\land E_2] = \Pr[E_2]\Pr[E_1|E_2] = \frac{\delta}{2}\Pr[E_1|E_2]$. Next, we fix arbitrary $i\in [k]$. Note that for each $a\in \mathbb F$, the marginal distribution of $Y_a$ is the uniform distribution over $\mathbb F^m$, thus, $\mathbb E[Y_a] = \Delta(\hat{\pi},\pi^*)$. As a result, $\mathbb E[\Delta(\hat{\pi}|_Y, \pi^*|_Y)]=\Delta(\hat{\pi},\pi^*)$. By Markov's inequality, we have that $\Pr[E_1|i]\le \frac14$ for every choice $i\in [k]$. Thus, we have that $\Pr[E_1|E_2] \le \frac14$. Hence $\Pr[E_1\land E_2]\le \frac{\delta}{8}$.

    Thus, with probability at least $\frac{\delta}8$, both $E_1$ and $E_2$ happen. Below, we show that in such cases, the query result is at least $\frac{1}{4}$-far from any accepting configuration. Thus, $\mathcal P$ has $\frac{\delta}2$-robust soundness $\le 1-\frac{\delta}8$.

    To show this, we first recall that the query result consists of two parts, each part has equal length $3|\mathbb F|\log |\mathbb F|$.
    \begin{itemize}
        \item The first part reads from $x_{{\rm copy},i,\cdot}$, which supposed to be a $3|\mathbb F|\log |\mathbb F|$-reptition of some $b\in \{0,1\}^t$.
        \item The second part reads from $\hat{\pi}|_Y$, where for each $a\in \mathbb F$, $\hat{\pi}(Y_a, \cdot)$ is supposed to be a codeword of ${\rm ECC}$, and $\{q(a) = {\rm Dec}(\hat{\pi}(Y_a, \cdot))\}_{a\in \mathbb F}$ is supposed to be a truth table of some univariate polynomial with parallel degree $mH$. Furthermore, $q(0)$ should equal $b$. Note that all accepting configuration in this part has relative distance $\ge \delta({\rm ECC})(1-\frac{mH}{|\mathbb F|})$.
    \end{itemize}
    
    Now, suppose both $E_1$ and $E_2$ happen, thus $\Delta(\hat{\pi}|_Y, \pi^*|_Y)\le 4\Delta(\hat{\pi},\pi^*)\le 4\delta$ and $i\in B$, which means that for at least $\frac12$ proportion choice of $j\in [3|\mathbb F|\log |\mathbb F|]$, $x_{{\rm copy}, i, j}\ne x_i^*$. Then, consider any accepting configuration for this test:
    \begin{itemize}
        \item If $b = x_i^*$, then this configuration differs with the query result on $\ge \frac12$ fraction of indices in the first part.
        \item If $b\ne x_i^*$, then this configuration differs with the query result on $\ge (\delta({\rm ECC})(1-\frac{mH}{|\mathbb F|})-4\delta)\ge \frac12$ fraction of indices in the second part.
    \end{itemize}
    Since both parts has the same length, we deduce that the query result is at least $\frac{1}{4}$-far from any accepting configuration.

    
\end{proof}


==> improve/prelim-backup.tex <==
\section{Preliminaries}\label{sec:prelim}

For a positive integer $n$, we use $[n]$ to denote the set $\cbra{1,2,\ldots,n}$.
We use $\log$ to denote the logarithm with base $2$.
For an event $\Ecal$, we use $\indicator_\Ecal$ as the indicator function, which equals $1$ if $\Ecal$ happens and equals $0$ if otherwise.
For a distribution $\mu$, we use $x\sim\mu$ to denote a sample from $\mu$ drawn under the distribution $\mu$. For a non-empty set $S$ of finite size, we use $x\sim S$ to denote a unifomly random element drawn from $S$.

For disjoint sets $S$ and $T$, we use $S\dot\cup T$ to denote their union while emphasizing $S\cap T=\emptyset$.
For a prime power $q=p^t$ where $p$ is a prime and $t\ge1$ is an integer, we use $\Fbb_q$ to denote the finite field of order $p^t$ and characteristic $p$.
We use superscript $\top$ to denote vector and matrix transpose. For two vectors $u,v\in\Fbb^d$, we use $\abra{u,v}$ to denote their inner product which equals $u^\top v$ (or $v^\top u$).
%For two matrices $A,B\in\Fbb^{d\times d}$, we use $\abra{A,B}=\sum_{i,j\in[d]}A_{i,j}B_{i,j}$ to denote their inner product.

\paragraph{Asymptotics}
Throughout the paper, we use $O(\cdot),\Theta(\cdot),\Omega(\cdot)$ to hide absolute constants that do not depend on any other parameter.

\subsection{Backgrounds in Coding Theory}

\paragraph{Word}
We say $x$ is a word (aka vector) with alphabet $\Sigma$ if $x$ is a string of finite length and each entry is an element from $\Sigma$.
Assume $x$ has length $m$. For each $I\subseteq[m]$, we use $x_I$ to denote the sub-string of $x$ on entries in $I$.
When $I=\cbra{i}$ is a singleton set, we simply use $x_i$ to denote $x_{\cbra{i}}$.

Let $y$ be another word with alphabet $\Sigma$. We use $x\circ y$ to denote the concatenation of $x$ and $y$.
If $y$ is also of length $m$, we define $\Delta(x,y) := \Pr_{i\in [m]}[x_i\ne y_i]$ as their relative Hamming distance.

Below, we define the error-correcting code.
\begin{definition}[Error Correcting Codes (ECCs)]\label{def:ecc}
An error correcting code is the image of the encoding map $C\colon\Sigma_1^k\to \Sigma_2^K$ with message length $k$, codeword length $K$. We say that the ECC has a relative distance $\delta$ if $\Delta(C(x),C(y))\ge \delta$ holds for any distinct $x,y\in\Sigma_1^k$. We use $\delta(C)$ to denote the relative distance of $C$.% $\rm{Im}(C)$ to denote the codewords of $C$. W
\end{definition}




\subsection{Backgrounds in Robust Probabilistic Checkable Proof of Proximity}

\paragraph{Pair Language and Robust PCPP}
We say $L$ is a pair language over the alphabet $\Sigma$ if all words of $L$ are in the form $(x,y)$ where $x,y\in \Sigma^*$. For each $x\in \Sigma^*$, we define $L(x)$ as $\{y\in \Sigma^*| (x,y)\in L\}$ as the restriction of $L$ on $x$.

For a word $y$ and a set $S$ of words, if $\Delta(x,y)>\delta$ holds for every $x\in S$, we say $y$ is $\delta$-far from $S$; otherwise we say $y$ is $\delta$-close to $S$.
We now rigorously define the notion of \emph{robust probabilistic checkable proof of proximity (robust PCPP)}.

\begin{definition}[Robust PCPP]\label{def:pcpp}
Given a pair language $L$ with alphabet $\Sigma$, a $(q, r, \rho, \delta, \varepsilon)$-robust PCPP verifier $\mathcal P$ takes as input a pair of words $(x,y)$ and an auxiliary proof $\pi$ with alphabet $\Sigma$, such that:
\begin{enumerate}[label=\textbf{(T\arabic*)}]
    \item \label{def-pcpp-procedure} The verifier $\mathcal P$ reads all bits of $x$, tosses at most $r(|x|)$ many unbiased coins, makes at most $q(|x|)$ queries on $y$ and $\pi$, and then decides to accept or reject within runtime $(|x|+\Sigma)^{O(1)}$. 
    
    We use $I_r$ to denote the query positions on $y\circ \pi$ under randomness $r$, and use $\mathcal P(x,y,r,a)$ to indicate the behavior (i.e., accept or reject) of $\mathcal P$ under randomness $r$ and query answer $a$.
    \item \label{def-pcpp-completeness} If $(x,y)\in L$, then there exists some $\pi$ such that $\mathcal P$ always accepts.
    \item \label{def-pcpp-robust-soundness} If $y$ is $\delta$-far from $L(x)$, then for every $\pi$, the probability that the query answer is $\rho$-close to an accepting configuration is at most $1-\varepsilon$, i.e., 
    $$
    \Pr_r[\exists a\in\Sigma^{I_r}\text{ such that }\mathcal P(x,y,r,a)\text{ accepts and }\Delta(a, (y\circ \pi)_{I_r})\le\rho]\le 1-\varepsilon.
    $$
    The probability $1-\varepsilon$ is also termed as the $\rho$-robust soundness.
\end{enumerate}
\end{definition}


\begin{remark}\label{rmk:pcpp}
We can always upper bound $|\pi|$ by $2^{r(|x|)}q(|x|)$, for which reason we do not put an additional parameter in \Cref{def:pcpp}.
\end{remark}

Below, we define several pair languages used in our paper.
First we fix the notation for words with vector-valued alphabet.
Let $x\in(\Sigma^t)^k$ be a word of length $k$ and alphabet $\Sigma^t$, where $t$ is defined as the dimension.
Let $i\in[k]$ and $j\in[t]$.
We use $x_i\in\Sigma^t$ to denote the $i$-th entry of $x$, use $x_i[j]\in\Sigma$ to denote the $j$-th coordinate of $x_i$, and use $x[j]\in\Sigma^k$ to denote $x_1[j]\circ x_2[j]\circ\cdots\circ x_k[j]$.

\paragraph{Parallel Circuit Value} 
Given a predicate $C:\bin^k\to \{0,1\}$, we say a word $x\in (\{0,1\}^t)^k$ parallel satisfies $C$ iff $C(x[j]) = 1$ holds for every coordinate $j\in[t]$.

\begin{definition}[\pcircuit{}]
\label{def:pcircuit}
    Given the dimension $t$, \pcircuit{} is a pair language over $\{0,1\}^t$ consisting of all words in the form of $(C,x)$, where:
    \begin{itemize}
        \item $C$ is a Boolean circuit\footnote{This circuit serves as a predicate and uses standard Boolean gates: AND/OR gate of fan-in two and fan-out unbounded, together with NOT gate of fan-out unbounded.} with $k$ input bits.
        \item $x\in (\{0,1\}^t)^k$ is a word that parallel satisfies $C$.
    \end{itemize}
We use {\sc CktVal} to denote \pcircuit{} with $t=1$.
\end{definition}

\iffalse

We list some known PCPP constructions for {\sc CktVal} and \pcircuit{}.

\begin{theorem}[ALMSS-type PCPP]
\label{thm:almss}
    For every $\delta\in (0,1)$, {\sc CktVal} has 
    $$
    \text{a $\pbra{(\log k)^{O(1)}, O(\log k),\Omega(\delta), \delta, \Omega(\delta)}$-robust PCPP verifier,}
    $$
    where $k$ is the size of the circuit $C$. \kewen{Add ref?}
\end{theorem}


\begin{theorem}[PCPPs for \pcircuit{} with Exponential Size, \cite{GLRSW24}]
\label{thm:pcpp-exp-circuit}
    For every $\delta \in (0, \frac1{800})$, \pcircuit{} has 
    $$
    \text{a $\pbra{4, O(k^2), \frac{1}{5}, \delta, 48\delta}$-robust PCPP verifier},
    $$
    where $k$ is the size of the circuit $C$. \kewen{Did we prove it's robust?}
    \xr{Randomness is $2^{k^2}$?}
\end{theorem}


\paragraph{Linear Equation System} A linear equation system is defined as follows. For each system $I$, we are given an integer $\ell$, the dimension $t$, $\ell$ matrices $M_1,\dots,M_{\ell}\in \mathbb F_2^{t\times t}$, and the coefficients $\{a_{i,j,k}\}_{i,j,k\in [\ell]}, \{b_{j,k}\}_{j,k\in [\ell]}$. This defines a set of linear constraints over $3\ell$ variables $c_1,\dots, c_{\ell}, x_1,\dots, x_{\ell}, \\y_1,\dots, y_{\ell}$, each variable has the alphabet $\mathbb F_2^t$. The constraints are:
\begin{equation}
\label{eq:sys}
    \forall i\in [\ell]\quad c_i = \sum_{j,k\in [\ell]}a_{i,j,k}M_jx_k+\sum_{j\in [\ell]}b_{i,j}y_j
\end{equation}

\begin{definition}[\lineq{}]
\label{def:lineq}
    Given the dimension $t$, \lineq{} is a pair language over $\{0,1\}^t$. It consists of all words in the form of $(I,(c,x,y))$, where:
    \begin{itemize}
        \item $I = (\ell, M_1,\dots,M_{\ell}, \{a_{i,j,k}\}_{i,j,k\in [\ell]}, \{b_{j,k}\}_{j,k\in [\ell]}$ that defines a set of linear constraints as \Cref{eq:sys}. 
        \item $c,x,y\in (\{0,1\}^t)^k$ is the solution of the system $I$.
    \end{itemize}
\end{definition}


\begin{theorem}[PCPPs for \lineq{} with Exponential Size, \cite{GLRSW24}]
    For every $\delta \in (0, \frac1{400})$, \lineq{} has
    $$
    \text{a $\pbra{4, O(\ell^2), \frac{1}{5}, \delta, 24\delta}$-robust PCPP verifier,}
    $$
    where the system has $3\ell$ variables. \kewen{Did we prove it's robust?s}
\end{theorem}
\fi

